Search for Doubly Charged Higgs Bosons with Lepton-Flavor-Violating Decays involving Tau Leptons

We search for pair production of doubly charged Higgs particles followed by decays into electron-tau and muon-tau pairs using data (350 inverse picobarns) collected from proton-antiproton collisions at 1.96 TeV by the CDF II experiment. We search separately for cases where three or four final-state leptons are detected, and combine results for exclusive decays to left-handed electron-tau (muon-tau) pairs. We set a lower mass limit of 114 (112) GeV/cc at the 95% confidence level for left-handed doubly charged Higgs.

==> authors.tex <==
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China} 
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439} 
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain} 
\affiliation{Baylor University, Waco, Texas  76798} 
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy} 
\affiliation{Brandeis University, Waltham, Massachusetts 02254} 
\affiliation{University of California, Davis, Davis, California  95616} 
\affiliation{University of California, Los Angeles, Los Angeles, California  90024} 
\affiliation{University of California, San Diego, La Jolla, California  92093} 
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106} 
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain} 
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213} 
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637} 
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia} 
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia} 
\affiliation{Duke University, Durham, North Carolina  27708} 
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510} 
\affiliation{University of Florida, Gainesville, Florida  32611} 
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy} 
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland} 
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom} 
\affiliation{Harvard University, Cambridge, Massachusetts 02138} 
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland} 
\affiliation{University of Illinois, Urbana, Illinois 61801} 
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218} 
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany} 
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea} 
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720} 
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom} 
\affiliation{University College London, London WC1E 6BT, United Kingdom} 
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain} 
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139} 
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7} 
\affiliation{University of Michigan, Ann Arbor, Michigan 48109} 
\affiliation{Michigan State University, East Lansing, Michigan  48824} 
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131} 
\affiliation{Northwestern University, Evanston, Illinois  60208} 
\affiliation{The Ohio State University, Columbus, Ohio  43210} 
\affiliation{Okayama University, Okayama 700-8530, Japan} 
\affiliation{Osaka City University, Osaka 588, Japan} 
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom} 
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy} 
\affiliation{LPNHE, Universite Pierre et Marie Curie/IN2P3-CNRS, UMR7585, Paris, F-75252 France} 
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104} 
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy} 
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260} 
\affiliation{Purdue University, West Lafayette, Indiana 47907} 
\affiliation{University of Rochester, Rochester, New York 14627} 
\affiliation{The Rockefeller University, New York, New York 10021} 
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy} 
\affiliation{Rutgers University, Piscataway, New Jersey 08855} 
\affiliation{Texas A\&M University, College Station, Texas 77843} 
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy} 
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan} 
\affiliation{Tufts University, Medford, Massachusetts 02155} 
\affiliation{Waseda University, Tokyo 169, Japan} 
\affiliation{Wayne State University, Detroit, Michigan  48201} 
\affiliation{University of Wisconsin, Madison, Wisconsin 53706} 
\affiliation{Yale University, New Haven, Connecticut 06520} 
\author{T.~Aaltonen}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{J.~Adelman}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{T.~Akimoto}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{M.G.~Albrow}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{B.~\'{A}lvarez~Gonz\'{a}lez}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{S.~Amerio}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{D.~Amidei}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{A.~Anastassov}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{A.~Annovi}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{J.~Antos}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{M.~Aoki}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{G.~Apollinari}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Apresyan}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{T.~Arisawa}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{A.~Artikov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{W.~Ashmanskas}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Attal}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{A.~Aurisano}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{F.~Azfar}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{P.~Azzi-Bacchetta}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{P.~Azzurri}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{N.~Bacchetta}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{W.~Badgett}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Barbaro-Galtieri}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{V.E.~Barnes}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{B.A.~Barnett}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218}
\author{S.~Baroiant}
\affiliation{University of California, Davis, Davis, California  95616}
\author{V.~Bartsch}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{G.~Bauer}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{P.-H.~Beauchemin}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{F.~Bedeschi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{P.~Bednar}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{S.~Behari}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218}
\author{G.~Bellettini}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{J.~Bellinger}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{A.~Belloni}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{D.~Benjamin}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{A.~Beretvas}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.~Beringer}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{T.~Berry}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{A.~Bhatti}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{M.~Binkley}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{D.~Bisello}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{I.~Bizjak}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{R.E.~Blair}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{C.~Blocker}
\affiliation{Brandeis University, Waltham, Massachusetts 02254}
\author{B.~Blumenfeld}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218}
\author{A.~Bocci}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{A.~Bodek}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{V.~Boisvert}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{G.~Bolla}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{A.~Bolshov}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{D.~Bortoletto}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{J.~Boudreau}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\author{A.~Boveia}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{B.~Brau}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{A.~Bridgeman}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{L.~Brigliadori}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{C.~Bromberg}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{E.~Brubaker}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{J.~Budagov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{H.S.~Budd}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{S.~Budd}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{K.~Burkett}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.~Busetto}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{P.~Bussey}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{A.~Buzatu}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{K.~L.~Byrum}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{S.~Cabrera$^r$}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{M.~Campanelli}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{M.~Campbell}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{F.~Canelli}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Canepa}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{D.~Carlsmith}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{R.~Carosi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{S.~Carrillo$^l$}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{S.~Carron}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{B.~Casal}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{M.~Casarsa}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Castro}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{P.~Catastini}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{D.~Cauz}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{M.~Cavalli-Sforza}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{A.~Cerri}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{L.~Cerrito$^p$}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{S.H.~Chang}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{Y.C.~Chen}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{M.~Chertok}
\affiliation{University of California, Davis, Davis, California  95616}
\author{G.~Chiarelli}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{G.~Chlachidze}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{F.~Chlebana}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{K.~Cho}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{D.~Chokheli}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{J.P.~Chou}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{G.~Choudalakis}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{S.H.~Chuang}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{K.~Chung}
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213}
\author{W.H.~Chung}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{Y.S.~Chung}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{C.I.~Ciobanu}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{M.A.~Ciocci}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{A.~Clark}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{D.~Clark}
\affiliation{Brandeis University, Waltham, Massachusetts 02254}
\author{G.~Compostella}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{M.E.~Convery}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.~Conway}
\affiliation{University of California, Davis, Davis, California  95616}
\author{B.~Cooper}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{K.~Copic}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{M.~Cordelli}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{G.~Cortiana}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{F.~Crescioli}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{C.~Cuenca~Almenar$^r$}
\affiliation{University of California, Davis, Davis, California  95616}
\author{J.~Cuevas$^o$}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{R.~Culbertson}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.C.~Cully}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{D.~Dagenhart}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Datta}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{T.~Davies}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{P.~de~Barbaro}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{S.~De~Cecco}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{A.~Deisher}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{G.~De~Lentdecker$^d$}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{G.~De~Lorenzo}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{M.~Dell'Orso}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{L.~Demortier}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{J.~Deng}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{M.~Deninno}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{D.~De~Pedis}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{P.F.~Derwent}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.P.~Di~Giovanni}
\affiliation{LPNHE, Universite Pierre et Marie Curie/IN2P3-CNRS, UMR7585, Paris, F-75252 France}
\author{C.~Dionisi}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{B.~Di~Ruzza}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{J.R.~Dittmann}
\affiliation{Baylor University, Waco, Texas  76798}
\author{M.~D'Onofrio}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{S.~Donati}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{P.~Dong}
\affiliation{University of California, Los Angeles, Los Angeles, California  90024}
\author{J.~Donini}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{T.~Dorigo}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{S.~Dube}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{J.~Efron}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{R.~Erbacher}
\affiliation{University of California, Davis, Davis, California  95616}
\author{D.~Errede}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{S.~Errede}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{R.~Eusebi}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{H.C.~Fang}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{S.~Farrington}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{W.T.~Fedorko}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{R.G.~Feild}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Feindt}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{J.P.~Fernandez}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{C.~Ferrazza}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{R.~Field}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{G.~Flanagan}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{R.~Forrest}
\affiliation{University of California, Davis, Davis, California  95616}
\author{S.~Forrester}
\affiliation{University of California, Davis, Davis, California  95616}
\author{M.~Franklin}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{J.C.~Freeman}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{I.~Furic}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{M.~Gallinaro}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{J.~Galyardt}
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213}
\author{F.~Garberson}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{J.E.~Garcia}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{A.F.~Garfinkel}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{K.~Genser}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{H.~Gerberich}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{D.~Gerdes}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{S.~Giagu}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{V.~Giakoumopolou$^a$}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{P.~Giannetti}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{K.~Gibson}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\author{J.L.~Gimmell}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{C.M.~Ginsburg}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{N.~Giokaris$^a$}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{M.~Giordani}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{P.~Giromini}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{M.~Giunta}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{V.~Glagolev}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{D.~Glenzinski}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Gold}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{N.~Goldschmidt}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{A.~Golossanov}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.~Gomez}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{G.~Gomez-Ceballos}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{M.~Goncharov}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{O.~Gonz\'{a}lez}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{I.~Gorelov}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{A.T.~Goshaw}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{K.~Goulianos}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{A.~Gresele}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{S.~Grinstein}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{C.~Grosso-Pilcher}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{R.C.~Group}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{U.~Grundler}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{J.~Guimaraes~da~Costa}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{Z.~Gunay-Unalan}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{C.~Haber}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{K.~Hahn}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{S.R.~Hahn}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{E.~Halkiadakis}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{A.~Hamilton}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{B.-Y.~Han}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{J.Y.~Han}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{R.~Handler}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{F.~Happacher}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{K.~Hara}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{D.~Hare}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{M.~Hare}
\affiliation{Tufts University, Medford, Massachusetts 02155}
\author{S.~Harper}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{R.F.~Harr}
\affiliation{Wayne State University, Detroit, Michigan  48201}
\author{R.M.~Harris}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Hartz}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\author{K.~Hatakeyama}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{J.~Hauser}
\affiliation{University of California, Los Angeles, Los Angeles, California  90024}
\author{C.~Hays}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{M.~Heck}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{A.~Heijboer}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{B.~Heinemann}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~Heinrich}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{C.~Henderson}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{M.~Herndon}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{J.~Heuser}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{S.~Hewamanage}
\affiliation{Baylor University, Waco, Texas  76798}
\author{D.~Hidas}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{C.S.~Hill$^c$}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{D.~Hirschbuehl}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{A.~Hocker}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{S.~Hou}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{M.~Houlden}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{S.-C.~Hsu}
\affiliation{University of California, San Diego, La Jolla, California  92093}
\author{B.T.~Huffman}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{R.E.~Hughes}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{U.~Husemann}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{J.~Huston}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{J.~Incandela}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{G.~Introzzi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{M.~Iori}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{A.~Ivanov}
\affiliation{University of California, Davis, Davis, California  95616}
\author{B.~Iyutin}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{E.~James}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{B.~Jayatilaka}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{D.~Jeans}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{E.J.~Jeon}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{S.~Jindariani}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{W.~Johnson}
\affiliation{University of California, Davis, Davis, California  95616}
\author{M.~Jones}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{K.K.~Joo}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{S.Y.~Jun}
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213}
\author{J.E.~Jung}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{T.R.~Junk}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{T.~Kamon}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{D.~Kar}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{P.E.~Karchin}
\affiliation{Wayne State University, Detroit, Michigan  48201}
\author{Y.~Kato}
\affiliation{Osaka City University, Osaka 588, Japan}
\author{R.~Kephart}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{U.~Kerzel}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{V.~Khotilovich}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{B.~Kilminster}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{D.H.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{H.S.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{J.E.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{M.J.~Kim}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{S.B.~Kim}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{S.H.~Kim}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{Y.K.~Kim}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{N.~Kimura}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{L.~Kirsch}
\affiliation{Brandeis University, Waltham, Massachusetts 02254}
\author{S.~Klimenko}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{M.~Klute}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{B.~Knuteson}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{B.R.~Ko}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{S.A.~Koay}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{K.~Kondo}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{D.J.~Kong}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{J.~Konigsberg}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{A.~Korytov}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{A.V.~Kotwal}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{J.~Kraus}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{M.~Kreps}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{J.~Kroll}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{N.~Krumnack}
\affiliation{Baylor University, Waco, Texas  76798}
\author{M.~Kruse}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{V.~Krutelyov}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{T.~Kubo}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.~E.~Kuhlmann}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{T.~Kuhr}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{N.P.~Kulkarni}
\affiliation{Wayne State University, Detroit, Michigan  48201}
\author{Y.~Kusakabe}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{S.~Kwang}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{A.T.~Laasanen}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{S.~Lai}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{S.~Lami}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{S.~Lammel}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Lancaster}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{R.L.~Lander}
\affiliation{University of California, Davis, Davis, California  95616}
\author{K.~Lannon}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{A.~Lath}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{G.~Latino}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{I.~Lazzizzera}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{T.~LeCompte}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{J.~Lee}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{J.~Lee}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{Y.J.~Lee}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{S.W.~Lee$^q$}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{R.~Lef\`{e}vre}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{N.~Leonardo}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{S.~Leone}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{S.~Levy}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{J.D.~Lewis}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{C.~Lin}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{C.S.~Lin}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~Linacre}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{M.~Lindgren}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{E.~Lipeles}
\affiliation{University of California, San Diego, La Jolla, California  92093}
\author{A.~Lister}
\affiliation{University of California, Davis, Davis, California  95616}
\author{D.O.~Litvintsev}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{T.~Liu}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{N.S.~Lockyer}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{A.~Loginov}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Loreti}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{L.~Lovas}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{R.-S.~Lu}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{D.~Lucchesi}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{J.~Lueck}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{C.~Luci}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{P.~Lujan}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{P.~Lukens}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.~Lungu}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{L.~Lyons}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{J.~Lys}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{R.~Lysak}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{E.~Lytken}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{P.~Mack}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{D.~MacQueen}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{R.~Madrak}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{K.~Maeshima}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{K.~Makhoul}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{T.~Maki}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{P.~Maksimovic}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218}
\author{S.~Malde}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{S.~Malik}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{G.~Manca}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{A.~Manousakis$^a$}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{F.~Margaroli}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{C.~Marino}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{C.P.~Marino}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{A.~Martin}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Martin}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218}
\author{V.~Martin$^j$}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{M.~Mart\'{\i}nez}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{R.~Mart\'{\i}nez-Ballar\'{\i}n}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{T.~Maruyama}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{P.~Mastrandrea}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{T.~Masubuchi}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{M.E.~Mattson}
\affiliation{Wayne State University, Detroit, Michigan  48201}
\author{P.~Mazzanti}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{K.S.~McFarland}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{P.~McIntyre}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{R.~McNulty$^i$}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{A.~Mehta}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{P.~Mehtala}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{S.~Menzemer$^k$}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{A.~Menzione}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{P.~Merkel}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{C.~Mesropian}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{A.~Messina}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{T.~Miao}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{N.~Miladinovic}
\affiliation{Brandeis University, Waltham, Massachusetts 02254}
\author{J.~Miles}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{R.~Miller}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{C.~Mills}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{M.~Milnik}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{A.~Mitra}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{G.~Mitselmakher}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{H.~Miyake}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.~Moed}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{N.~Moggi}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{C.S.~Moon}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{R.~Moore}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Morello}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{P.~Movilla~Fernandez}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~M\"ulmenst\"adt}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{A.~Mukherjee}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{Th.~Muller}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{R.~Mumford}
\affiliation{The Johns Hopkins University, Baltimore, Maryland 21218}
\author{P.~Murat}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Mussini}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{J.~Nachtman}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{Y.~Nagai}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{A.~Nagano}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{J.~Naganoma}
\affiliation{Waseda University, Tokyo 169, Japan}
\author{K.~Nakamura}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{I.~Nakano}
\affiliation{Okayama University, Okayama 700-8530, Japan}
\author{A.~Napier}
\affiliation{Tufts University, Medford, Massachusetts 02155}
\author{V.~Necula}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{C.~Neu}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{M.S.~Neubauer}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{J.~Nielsen$^f$}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{L.~Nodulman}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{M.~Norman}
\affiliation{University of California, San Diego, La Jolla, California  92093}
\author{O.~Norniella}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{E.~Nurse}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{S.H.~Oh}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{Y.D.~Oh}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{I.~Oksuzian}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{T.~Okusawa}
\affiliation{Osaka City University, Osaka 588, Japan}
\author{R.~Oldeman}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{R.~Orava}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{K.~Osterberg}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{S.~Pagan~Griso}
\affiliation{University of Padova, Istituto Nazionale di Fisica Nucleare, Sezione di Padova-Trento, I-35131 Padova, Italy}
\author{C.~Pagliarone}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{E.~Palencia}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{V.~Papadimitriou}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Papaikonomou}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{A.A.~Paramonov}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{B.~Parks}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{S.~Pashapour}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{J.~Patrick}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.~Pauletta}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{M.~Paulini}
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213}
\author{C.~Paus}
\affiliation{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139}
\author{D.E.~Pellett}
\affiliation{University of California, Davis, Davis, California  95616}
\author{A.~Penzo}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{T.J.~Phillips}
\affiliation{Duke University, Durham, North Carolina  27708}
\author{G.~Piacentino}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{J.~Piedra}
\affiliation{LPNHE, Universite Pierre et Marie Curie/IN2P3-CNRS, UMR7585, Paris, F-75252 France}
\author{L.~Pinera}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{K.~Pitts}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{C.~Plager}
\affiliation{University of California, Los Angeles, Los Angeles, California  90024}
\author{L.~Pondrom}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{X.~Portell}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{O.~Poukhov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{N.~Pounder}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{F.~Prakoshyn}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{A.~Pronko}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.~Proudfoot}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{F.~Ptohos$^h$}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.~Punzi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{J.~Pursley}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{J.~Rademacker$^c$}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{A.~Rahaman}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\author{V.~Ramakrishnan}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{N.~Ranjan}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{I.~Redondo}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{B.~Reisert}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{V.~Rekovic}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{P.~Renton}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{M.~Rescigno}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{S.~Richter}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{F.~Rimondi}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\author{L.~Ristori}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{A.~Robson}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{T.~Rodrigo}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{E.~Rogers}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{S.~Rolli}
\affiliation{Tufts University, Medford, Massachusetts 02155}
\author{R.~Roser}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.~Rossi}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{R.~Rossin}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{P.~Roy}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{A.~Ruiz}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{J.~Russ}
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213}
\author{V.~Rusu}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{H.~Saarikko}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{A.~Safonov}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{W.K.~Sakumoto}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{G.~Salamanna}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{O.~Salt\'{o}}
\affiliation{Institut de Fisica d'Altes Energies, Universitat Autonoma de Barcelona, E-08193, Bellaterra (Barcelona), Spain}
\author{L.~Santi}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{S.~Sarkar}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{L.~Sartori}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{K.~Sato}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Savoy-Navarro}
\affiliation{LPNHE, Universite Pierre et Marie Curie/IN2P3-CNRS, UMR7585, Paris, F-75252 France}
\author{T.~Scheidle}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{P.~Schlabach}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{E.E.~Schmidt}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{M.A.~Schmidt}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{M.P.~Schmidt}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Schmitt}
\affiliation{Northwestern University, Evanston, Illinois  60208}
\author{T.~Schwarz}
\affiliation{University of California, Davis, Davis, California  95616}
\author{L.~Scodellaro}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{A.L.~Scott}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{A.~Scribano}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{F.~Scuri}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{A.~Sedov}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{S.~Seidel}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{Y.~Seiya}
\affiliation{Osaka City University, Osaka 588, Japan}
\author{A.~Semenov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{L.~Sexton-Kennedy}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.~Sfyrla}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{S.Z.~Shalhout}
\affiliation{Wayne State University, Detroit, Michigan  48201}
\author{M.D.~Shapiro}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{T.~Shears}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{P.F.~Shepard}
\affiliation{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\author{D.~Sherman}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{M.~Shimojima$^n$}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{M.~Shochet}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{Y.~Shon}
\affiliation{University of Wisconsin, Madison, Wisconsin 53706}
\author{I.~Shreyber}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{A.~Sidoti}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{P.~Sinervo}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{A.~Sisakyan}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{A.J.~Slaughter}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.~Slaunwhite}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{K.~Sliwa}
\affiliation{Tufts University, Medford, Massachusetts 02155}
\author{J.R.~Smith}
\affiliation{University of California, Davis, Davis, California  95616}
\author{F.D.~Snider}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{R.~Snihur}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{M.~Soderberg}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{A.~Soha}
\affiliation{University of California, Davis, Davis, California  95616}
\author{S.~Somalwar}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{V.~Sorin}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{J.~Spalding}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{F.~Spinella}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{T.~Spreitzer}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{P.~Squillacioti}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{M.~Stanitzki}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{R.~St.~Denis}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{B.~Stelzer}
\affiliation{University of California, Los Angeles, Los Angeles, California  90024}
\author{O.~Stelzer-Chilton}
\affiliation{University of Oxford, Oxford OX1 3RH, United Kingdom}
\author{D.~Stentz}
\affiliation{Northwestern University, Evanston, Illinois  60208}
\author{J.~Strologas}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{D.~Stuart}
\affiliation{University of California, Santa Barbara, Santa Barbara, California 93106}
\author{J.S.~Suh}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{A.~Sukhanov}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{H.~Sun}
\affiliation{Tufts University, Medford, Massachusetts 02155}
\author{I.~Suslov}
\affiliation{Joint Institute for Nuclear Research, RU-141980 Dubna, Russia}
\author{T.~Suzuki}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{A.~Taffard$^e$}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{R.~Takashima}
\affiliation{Okayama University, Okayama 700-8530, Japan}
\author{Y.~Takeuchi}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{R.~Tanaka}
\affiliation{Okayama University, Okayama 700-8530, Japan}
\author{M.~Tecchio}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{P.K.~Teng}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{K.~Terashi}
\affiliation{The Rockefeller University, New York, New York 10021}
\author{J.~Thom$^g$}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{A.S.~Thompson}
\affiliation{Glasgow University, Glasgow G12 8QQ, United Kingdom}
\author{G.A.~Thompson}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{E.~Thomson}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{P.~Tipton}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{V.~Tiwari}
\affiliation{Carnegie Mellon University, Pittsburgh, PA  15213}
\author{S.~Tkaczyk}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{D.~Toback}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{S.~Tokar}
\affiliation{Comenius University, 842 48 Bratislava, Slovakia; Institute of Experimental Physics, 040 01 Kosice, Slovakia}
\author{K.~Tollefson}
\affiliation{Michigan State University, East Lansing, Michigan  48824}
\author{T.~Tomura}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{D.~Tonelli}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{S.~Torre}
\affiliation{Laboratori Nazionali di Frascati, Istituto Nazionale di Fisica Nucleare, I-00044 Frascati, Italy}
\author{D.~Torretta}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{S.~Tourneur}
\affiliation{LPNHE, Universite Pierre et Marie Curie/IN2P3-CNRS, UMR7585, Paris, F-75252 France}
\author{W.~Trischuk}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{Y.~Tu}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{N.~Turini}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{F.~Ukegawa}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.~Uozumi}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki 305, Japan}
\author{S.~Vallecorsa}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{N.~van~Remortel}
\affiliation{Division of High Energy Physics, Department of Physics, University of Helsinki and Helsinki Institute of Physics, FIN-00014, Helsinki, Finland}
\author{A.~Varganov}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{E.~Vataga}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{F.~V\'{a}zquez$^l$}
\affiliation{University of Florida, Gainesville, Florida  32611}
\author{G.~Velev}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{C.~Vellidis$^a$}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{V.~Veszpremi}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{M.~Vidal}
\affiliation{Centro de Investigaciones Energeticas Medioambientales y Tecnologicas, E-28040 Madrid, Spain}
\author{R.~Vidal}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{I.~Vila}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{R.~Vilar}
\affiliation{Instituto de Fisica de Cantabria, CSIC-University of Cantabria, 39005 Santander, Spain}
\author{T.~Vine}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{M.~Vogel}
\affiliation{University of New Mexico, Albuquerque, New Mexico 87131}
\author{I.~Volobouev$^q$}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{G.~Volpi}
\affiliation{Istituto Nazionale di Fisica Nucleare Pisa, Universities of Pisa, Siena and Scuola Normale Superiore, I-56127 Pisa, Italy}
\author{F.~W\"urthwein}
\affiliation{University of California, San Diego, La Jolla, California  92093}
\author{P.~Wagner}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{R.G.~Wagner}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{R.L.~Wagner}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.~Wagner-Kuhr}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{W.~Wagner}
\affiliation{Institut f\"{u}r Experimentelle Kernphysik, Universit\"{a}t Karlsruhe, 76128 Karlsruhe, Germany}
\author{T.~Wakisaka}
\affiliation{Osaka City University, Osaka 588, Japan}
\author{R.~Wallny}
\affiliation{University of California, Los Angeles, Los Angeles, California  90024}
\author{S.M.~Wang}
\affiliation{Institute of Physics, Academia Sinica, Taipei, Taiwan 11529, Republic of China}
\author{A.~Warburton}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{D.~Waters}
\affiliation{University College London, London WC1E 6BT, United Kingdom}
\author{M.~Weinberger}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{W.C.~Wester~III}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{B.~Whitehouse}
\affiliation{Tufts University, Medford, Massachusetts 02155}
\author{D.~Whiteson$^e$}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{A.B.~Wicklund}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{E.~Wicklund}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{G.~Williams}
\affiliation{Institute of Particle Physics: McGill University, Montr\'{e}al, Canada H3A~2T8; and University of Toronto, Toronto, Canada M5S~1A7}
\author{H.H.~Williams}
\affiliation{University of Pennsylvania, Philadelphia, Pennsylvania 19104}
\author{P.~Wilson}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{B.L.~Winer}
\affiliation{The Ohio State University, Columbus, Ohio  43210}
\author{P.~Wittich$^g$}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{S.~Wolbers}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{C.~Wolfe}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{T.~Wright}
\affiliation{University of Michigan, Ann Arbor, Michigan 48109}
\author{X.~Wu}
\affiliation{University of Geneva, CH-1211 Geneva 4, Switzerland}
\author{S.M.~Wynne}
\affiliation{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\author{A.~Yagil}
\affiliation{University of California, San Diego, La Jolla, California  92093}
\author{K.~Yamamoto}
\affiliation{Osaka City University, Osaka 588, Japan}
\author{J.~Yamaoka}
\affiliation{Rutgers University, Piscataway, New Jersey 08855}
\author{T.~Yamashita}
\affiliation{Okayama University, Okayama 700-8530, Japan}
\author{C.~Yang}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{U.K.~Yang$^m$}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{Y.C.~Yang}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{W.M.~Yao}
\affiliation{Ernest Orlando Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{G.P.~Yeh}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.~Yoh}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{K.~Yorita}
\affiliation{Enrico Fermi Institute, University of Chicago, Chicago, Illinois 60637}
\author{T.~Yoshida}
\affiliation{Osaka City University, Osaka 588, Japan}
\author{G.B.~Yu}
\affiliation{University of Rochester, Rochester, New York 14627}
\author{I.~Yu}
\affiliation{Center for High Energy Physics: Kyungpook National University, Daegu 702-701, Korea; Seoul National University, Seoul 151-742, Korea; Sungkyunkwan University, Suwon 440-746, Korea; Korea Institute of Science and Technology Information, Daejeon, 305-806, Korea; Chonnam National University, Gwangju, 500-757, Korea}
\author{S.S.~Yu}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{J.C.~Yun}
\affiliation{Fermi National Accelerator Laboratory, Batavia, Illinois 60510}
\author{L.~Zanello}
\affiliation{Istituto Nazionale di Fisica Nucleare, Sezione di Roma 1, University of Rome ``La Sapienza," I-00185 Roma, Italy}
\author{A.~Zanetti}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Trieste/\ Udine, Italy}
\author{I.~Zaw}
\affiliation{Harvard University, Cambridge, Massachusetts 02138}
\author{X.~Zhang}
\affiliation{University of Illinois, Urbana, Illinois 61801}
\author{Y.~Zheng$^b$}
\affiliation{University of California, Los Angeles, Los Angeles, California  90024}
\author{S.~Zucchelli}
\affiliation{Istituto Nazionale di Fisica Nucleare, University of Bologna, I-40127 Bologna, Italy}
\collaboration{CDF Collaboration\footnote{With visitors from $^a$University of Athens, 15784 Athens, Greece, 
$^b$Chinese Academy of Sciences, Beijing 100864, China, 
$^c$University of Bristol, Bristol BS8 1TL, United Kingdom, 
$^d$University Libre de Bruxelles, B-1050 Brussels, Belgium, 
$^e$University of California Irvine, Irvine, CA  92697, 
$^f$University of California Santa Cruz, Santa Cruz, CA  95064, 
$^g$Cornell University, Ithaca, NY  14853, 
$^h$University of Cyprus, Nicosia CY-1678, Cyprus, 
$^i$University College Dublin, Dublin 4, Ireland, 
$^j$University of Edinburgh, Edinburgh EH9 3JZ, United Kingdom, 
$^k$University of Heidelberg, D-69120 Heidelberg, Germany, 
$^l$Universidad Iberoamericana, Mexico D.F., Mexico, 
$^m$University of Manchester, Manchester M13 9PL, England, 
$^n$Nagasaki Institute of Applied Science, Nagasaki, Japan, 
$^o$University de Oviedo, E-33007 Oviedo, Spain, 
$^p$Queen Mary, University of London, London, E1 4NS, England, 
$^q$Texas Tech University, Lubbock, TX  79409, 
$^r$IFIC(CSIC-Universitat de Valencia), 46071 Valencia, Spain, 
}}
\noaffiliation

